Towards Using Probabilistic Models to Design Software Systems with Inherent Uncertainty

The adoption of machine learning (ML) components in software systems raises new engineering challenges. In particular, the inherent uncertainty regarding functional suitability and the operation environment makes architecture evaluation and trade-off analysis difficult. We propose a software architecture evaluation method called Modeling Uncertainty During Design (MUDD) that explicitly models the uncertainty associated to ML components and evaluates how it propagates through a system. The method supports reasoning over how architectural patterns can mitigate uncertainty and enables comparison of different architectures focused on the interplay between ML and classical software components. While our approach is domain-agnostic and suitable for any system where uncertainty plays a central role, we demonstrate our approach using as example a perception system for autonomous driving.

==> arch_patterns.tex <==
\section{Using Architectural Patterns to Mitigate Uncertainty}
\label{sec:patterns}

Following the results from Section~\ref{sec:quantifying} and the changes suggested in Section~\ref{sec:qualitative}, we evaluate the impact of using architectural design patterns that can decrease stochastic uncertainty in depth estimation.
In particular, we explore the use of LIDAR~--~as suggested in~\cite{serban2018standard, behere2016functional}~--~to complement computer vision for depth estimation.
LIDAR is known to be more reliable than camera sensors and is explored by many autonomous vehicle manufacturers.
%
\begin{figure}[t]
 \centering
 \subfloat[End-to-end architecture.\label{fig:lidar_end}]{\includegraphics[width=5cm, keepaspectratio]{figures/lidar2.pdf}}
 \qquad 	\qquad 	\qquad
 \subfloat[Component-based architecture.\label{fig:lidar_dist}]{\includegraphics[width=5cm, keepaspectratio]{figures/lidar1.pdf}}
 \caption{Functional architectures when using the n-version programming pattern to reduce uncertainty for depth estimation.}
 \label{fig:lidar_both}
\end{figure}
%
 \begin{figure*}[t]
 	\centering
 	
 	\subfloat[Influence of stochastic uncertainty for depth estimation on planning.\label{fig:plot3}]{\includegraphics[width=5.9cm, keepaspectratio]{figures/bounds3}}
 	\quad
 	\subfloat[Influence of stochastic uncertainty for depth estimation and all epistemic uncertainties on planning. \label{fig:plot4}]{\includegraphics[width=5.9cm, keepaspectratio]{figures/bounds4}}
 	\caption{Quantitative evaluation of uncertainty in software architecture design using the n-version programming pattern.}
 	\label{fig:comparison_2}
 \end{figure*}
 %
As discussed in Section~\ref{sec:qualitative}, the output of depth estimation is independent for both architectures.
Therefore, the impact of adding a new component is the same for both designs.
Moreover, since the system we study is safety critical,  the integration of LIDAR can be done using architectural patterns for safety critical systems~\cite{armoush2010design}.
In particular, we evaluate the use of the \emph{n-versioning programming} pattern because it does not require any acceptance test.
The development of acceptance tests for \ac{DL} components is out of the scope of this paper.

The proposed changes are illustrated in Figure~\ref{fig:lidar_both}. 
The Voter component in Figure~\ref{fig:lidar_end} is illustrated next to depth estimation, although all inference tasks for the \ac{DL} components are performed at the same time.
Before the outcome of depth estimation is sent to planning, it is checked against the outcome of LIDAR.
Similarly, in the architecture from Figure~\ref{fig:lidar_dist}, the Voter component is added after depth estimation because all \ac{DL} components are independent.
 
The probability tables have to be adjusted as follows. 
Because LIDAR has high accuracy, its uncertainty only depends on the distance we want to perform analysis for~\cite{wang2017pedestrian}.
Since we do not have access to a LIDAR component, we use a proxy from literature~\cite{zhang2014loam} for its uncertainty values. 
The probability that the voter will be uncertain is a weighted average between the LIDAR and  the number of times depth estimation has low error rate and low uncertainty (according to the thresholds introduced in the previous section), where the LIDAR component's contribution is of $90\%$.
The final values are $0.09$ in the first case and $0.1$ in the second case. 
The formalism of \acp{BN} allows prior information to be incomplete. 
Therefore this approximation is sufficient to perform the same computations as in the previous section and evaluate the design alternatives.

The results are presented in Figure~\ref{fig:plot3} for the end-to-end architecture and Figure~\ref{fig:plot4} for the component-based architecture.
 We observe that in both cases, the component-based architecture is significantly more resilient to uncertainty, even for high values of epistemic uncertainty (Figure~\ref{fig:plot4}).
 A striking difference between the two designs is that the end-to-end architecture has a slight exponential curve for high levels of uncertainty while the component-based architecture has a linear and slightly logarithmic curve for high levels of uncertainty.
 
 When comparing the results before and after applying the n-version programming pattern (Figure~\ref{fig:comparison_2} and Figure~\ref{fig:variance}), we observe that applying the pattern is successful in decreasing the uncertainty influence on planning.
 Particularly for the component-based architecture, where the decrease is more significant than for the end-to-end architecture.

% Overall, the component based architecture is more resilient to uncertainty and more flexible to changes.
 

 

==> bayesian.tex <==
\section{Uncertainty Sources and Bayesian Networks}
\label{sec:bayesian}


Perez-Palacin and Mirandola~\cite{perez2014uncertainties} and Esfahani and Malek~\cite{esfahani2013uncertainty} discuss multiple sources of uncertainty to be considered in the context of self-adaptation.
Although many uncertainty sources are valid at design time, we are particularly interested in the uncertainty related to ``automated learning''~\cite{garlan2010software, weyns2017perpetual,mahdavi2017classification}, \ie~the inherent uncertainty related to \ac{ML} components.

In particular, we are interested in the uncertainty related to properties of \ac{ML} components that are impossible to fully verify before deployment, \ie~(1) the ability of a \ac{ML} component to always satisfy its intended functionality and (2) to cope with stochastic events in the operational environment.
According to~\cite{perez2014uncertainties} these sources of uncertainty can be classified by nature in:
%
\begin{itemize}
	\item \emph{\ac{EU}}~-~captures our ignorance of the correct model that generates the data. If the training data  for a \ac{ML} component does not accurately represent the data generation distribution, the model will have high epistemic uncertainty.
	This uncertainty can be removed given enough training data. However, the bounds on the training data set size needed to learn complex tasks, \eg~object recognition, are not achievable in practice.
	\item\emph{\ac{SU}}~-~captures the response of a \ac{ML} component to stochastic noise in the operational environment (\eg~noise in the observations). This uncertainty can not be removed with more training data.
\end{itemize}	
\noindent
% These two classes of uncertainty are well known in statistics and recognized as decision drivers in evaluating quality attributes of software using \ac{ML} components~\cite{salay2018using}.
% Moreover, they are well known the general \ac{ML} community, where the goal is to measure them accurately~\cite{kendall2017uncertainties}.

We propose to use these two sources of uncertainty as architectural design elements, in order to evaluate design alternatives for systems using \ac{ML} components.
% As mentioned in Section~\ref{sec:intro} and~\ref{sec:backcground}, we follow a bottom-up approach where uncertainty is evaluated in isolation~--~as it impacts specific \ac{ML} components~--~and as it propagates inside a system and influences other components.
%
For modeling a software system we use the structure and formalism of \acp{BN} because they allow to express beliefs (or incomplete prior information) about a variable and evaluate its influence on other connected variables.
Briefly, \acp{BN} are directed, acyclic graphs, that model a set of variables and their conditional dependencies. 
This model offers both a quantitative and a qualitative method to reason about a set of variables.
The former, qualitative, analysis uses the topological structure of the \ac{BN} where variables are represented as nodes of a graph and the dependencies between them as directed edges.

The latter, quantitative, analysis consists of specifying the conditional probability distributions (or tables in the discrete case) between dependent variables in the graph.
Since a \ac{BN} contains all assumptions about a model (the graphical structure, the conditional probabilities and other parameters), it has no hidden assumptions about inference rules.
The network's structure defines a joint probability model where the rules of probability calculus enable conclusions based on observations.
Probabilistic inference computes posterior probabilities for unobserved variables given observations of other variables in the model.
Due to space constraints, we delegate the formal introduction to \acp{BN} to~\cite{pearl2014probabilistic}.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

% TODO: make a distinction between machine learning and deep learning

Three assumptions underline the method presented above: (1) a functional architecture of a system exists, (2)  uncertainty measures can be extracted from the \ac{ML} components used and (3)  no cycles can occur in the graph (\acp{BN} are directed, acyclic graphs).
In this section we discuss the implications of these assumptions and present solutions that can be applied to more general cases. %ncrease the generalization of the method presented.
Moreover, we discuss the suitability of uncertainty as an element for architectural design and speculate on suitable alternatives.

As mention in Section~\ref{sec:modeling}, the space available to reason about quality properties of \ac{ML} components is smaller than other types of software components because the internal representation of complex \ac{ML} models can not be translated to a state-machine, has no causal structure and is generally opaque to humans.
Moreover, \ac{ML} algorithms provide approximate solutions, and not optimal.
For some algorithms and data (typically if the data is linearly separable) optimal criteria can be proven formally and achieved in practice~\cite{vapnik1998statistical}.
However, for complex tasks such as object recognition or image segmentation, where complicated relationships between the input variables need to be uncovered, theoretical settings suggest an optimal sample complexity that is currently beyond reach~\cite{schmidt2018adversarially}.
Some approximate solutions may satisfy the desired quality properties of a system, while others may not.
Testing quality attributes for \ac{ML} models proves difficult and is an ongoing research topic~\cite{szegedy2013intriguing,hendrycks2019benchmarking}.
Assuming that a functional architecture of a system exists is a minimal requirement; as it only requires to represent the desired goal (functionality) of a component and its interactions.
No other assumptions about the \ac{ML} algorithm used are needed.
The method introduced in this paper supports the design of safety critical systems, where functional architectural design is mandatory (see, for example, ISO 26262~\cite{iso26262}).
If a functional architecture does not exist, recovering it from software artifacts or creating it from scratch should be straight forward for most systems.
% TODO: say a bit more / draw conclusion
Therefore, the lack of a functional model is not a threat to the method.

% TODO: talk about uncertainty at the final distribution - which are not alright
Two elements are used in this paper to reason about a trained \ac{ML} model: its parameters and the final layer (which typically translates to a probability mass or density function).
We use uncertainty estimates as a proxy to evaluate if a \ac{ML} model is fit for a task and if stochasticity of the environment can affect the model's outcome.
However, none of this methods is exact and should not be considered a silver bullet.
One of the methods used in this paper requires dropout to approximate epistemic uncertainty, which might not used in some neural network architectures (\eg~ResNet) or other algorithms.
Using other methods to approximate uncertainties, such as bootstrapping, is a viable alternative~\cite{osband2016risk}.
The versatility of \acp{BN} makes it possible to also populate the networks by expert opinion and later refine the beliefs with data.
Therefore, concrete estimates of uncertainties are not a must to apply this method.
% TODO: maybe improve argumentation


In some cases several components will exchange information between themselves, thus forming cyclic dependencies.
In the current form, \acp{BN} do not allow cycles in conditional probabilities.
Formal generalizations of this model to cyclic or undirected graphs are available theoretically as Markov random fields or factor graphs~\cite{barber2012bayesian}.
Hybrid models use the best of both worlds, combining directed and undirected graphs~\cite{freno2011hybrid}.
Such models are a good fit to represent components that interact between themselves using undirected edges and components where the data flow is unidirectional using directed arrows.
Given the space constraints, we delegate the task of explicitly modeling such a system to future work.
It is worth noting that both the theoretical support and the practical implementations (\eg~software frameworks) are available.
% If two components exhcange data, they can be considered as an edge in a markov random field diagram and they can exchange uncertain
% data


% Talk about explainability as an alternative?
Causal reasoning, interpretable or explainable models are considered viable methods to increase the suitability of an algorithm for a task and the probability to satisfy its intended functionality.
Causal reasoning supports this goal by finding relations between a cause and effects; and is closer to the way human beings reason.
For example, in object recognition, identifying 4 wheels in an image may be the cause for the presence of a transportation device.
%This capability is lacking from current models and causal reasoning  can help to
Causal reasoning can decrease both epistemic and stochastic uncertainty.
Using cause-effect relationships helps humans beings learn from few examples and generalize to new instances relatively fast~\cite{pearl2000causality}.
However, causal reasoning is limited to hand-designed models or relatively small data-driven models and it is not yet suitable for complex tasks such as scene understanding.

Finding post-hoc explanations to decisions is also a popular research field; where \ac{ML} models are asked to provide some information to support their choices.
Many times, the information is based on the contribution of the input space to a task.
Data coming from algorithms that explain decisions can be embedded in the method presented above.
For example, the explanation confidence can be used as a different variable in the graph.
However, post-hoc explanations do not account for decision rules in making predictions and does not ensure accuracy in decisions or suitability for a task.
Lastly, using interpretable models is desired for every task, however, such models do not scale to complicated tasks such as object detection or semantic segmentation.
Therefore, the models currently used for such tasks are complex, not easy to interpret and subject to uncertainty.
% TODO: maybe say 'so what?'


% because cause-effect relationships should decrease the sample complexity needed to remove epistemic uncertainty and strengthen the model's response to stochastic events in the environment.
%Human beings can approximate



% 2. Position work in relation to patterns, as discussed in serban

==> figures/lidar_uncertainty.tex <==
\begin{figure}[h]
			\begin{tikzpicture}
					\tikzset{vertex/.style = {shape=circle,draw,minimum size=1.5em}}
					\tikzset{rect/.style = {shape=rectangle,draw,minimum size=1.5em}}			
					\tikzset{edge/.style = {->,> = latex'}}
										
					\node[rect] (camera) at (-3,6){camera};
					\node[vertex] (segmentation) at (2, 8) {seg.};
					\node[vertex] (epseg) at (0.5, 8.5) {epseg.};
					\node[vertex] (stseg) at (3.5, 8.5) {stseg.};		
					\node[vertex] (geometry) at (2, 6) {geo.};
					\node[vertex] (epgeo) at (-1, 4.5) {epgeo.};
					\node[vertex] (stgeo) at (-1, 7.5) {stgeo.};				
					\node[vertex] (localization) at (2, 4) {loc};
					\node[vertex] (eploc) at (0.5, 3.5) {eploc};
					\node[vertex] (stloc) at (3.5, 3.5) {stloc};				
					\node[vertex] (planning) at (4, 6) {plan};
					\node[vertex] (lidar) at (5, 6) {lidar};
										
					\draw[edge][bend right=15] (camera) to (segmentation);
					\draw[edge] (camera) to (geometry);
					\draw[edge][bend left=15] (camera) to (localization);
					
					\draw[edge] (localization) to (planning);
					\draw[edge] (geometry) to (planning);
					\draw[edge] (segmentation) to (planning);
					
					\draw[edge] (epseg) to (segmentation);
					\draw[edge] (stseg) to (segmentation);
					\draw[edge] (epgeo) to (geometry);
					\draw[edge] (stgeo) to (geometry);
					\draw[edge] (stloc) to (localization);
					\draw[edge] (eploc) to (localization);									
								
	\end{tikzpicture}
	\caption{Caption Missing}
	\label{fig:lidar}
\end{figure}



==> qualitative.tex <==
\section{Qualitative Architecture Evaluation}
\label{sec:qualitative}

Qualitatively, the  annotated functional architectures from Figure~\ref{fig:normal_unc} allow high level reasoning about threats  to the intended functionality coming from inherent uncertainty.
Nonetheless, the analysis is not limited to possible faults from uncertainty.
Other quality properties, \eg~availability, can be assessed similarly.

In order to evaluate design alternatives qualitatively, architects can apply well known evaluation methods such as questioning techniques, scenarios or check-lists~\cite{dobrica2002survey}.
We develop an example of scenario-based analysis; a technique systematized in~\cite{kazman2000toward}.
Scenarios analyze a use case or a change in a system.
The change can describe how one or more components perform an activity, the impact of adding another component to perform the same (or another) activity, the impact of adding a connection between existing components or any composition of these factors.
Describing the changes that are needed for a scenario is a qualitative method of architecture evaluation~\cite{dobrica2002survey}.

We analyze the scenario where high stochastic uncertainty in depth estimation leads to unsafe planning.
From Figure~\ref{fig:normal_unc} we can see that in the end-to-end architecture depth estimation is linked to semantic segmentation.
Stochastic uncertainty can not be removed using more training data, as indicated in Section~\ref{sec:bayesian}.
Therefore, the alternatives are to use a different training objective or a different \ac{ML} model altogether.
However, since the  scene understanding system is trained end-to-end, the new objective (or new model) can impact the internal representation of both segmentation and localization, which might increase their epistemic uncertainty and ultimately lead to unsafe planning.

In the component-based architecture depth estimation is only linked to planning.
Therefore, high stochastic uncertainty in depth estimation can be treated in isolation, by either deploying a new \ac{DL} component or using heterogeneous implementations to increase its confidence.
If the model is replaced, it will have no impact on the other components in the system.
In this case, the change requires less effort than in the end-to-end architecture because changing the depth estimation component does not require to change or re-train other components.


We also analyze the use of LIDAR~--~as suggested in~\cite{serban2018standard, behere2016functional}~--~to increase confidence in depth estimation and adopt the n-version programming pattern for safety critical systems to integrate it.
The change consists in adding a new LIDAR component and a voting mechanism between the \ac{DL} depth estimation component and the new  LIDAR component~\cite{armoush2010design}.
An illustration is provided in Figure~\ref{fig:lidar_both} and a more thorough discussion follows in Section~\ref{sec:patterns}.
For both architectures, the output of the \ac{DL} depth estimation components can be interpreted independently.
Therefore, deploying the new components specific to LIDAR will have the same impact for both architectures.
From the perspective of this change, both design alternatives are equivalent.
However, the component-based architecture still has a flexibility advantage when changing an individual component.

During qualitative evaluation, it is important that different stakeholders and roles responsible for parts of the system participate.
Such stakeholders may be algorithm developers, system and safety engineers or software architects.
We can see that by explicitly modeling of uncertainty at design time, a broader community of practitioners can participate in design decisions, even though the domain knowledge needed to understand the inner workings of \ac{ML} algorithms is not wide-spread.
% an advantage of elevating the problem at design time mentioned in~\cite{serban2019designing}.
%
In the following section we show how the same model enriched with quantitative measurements can be used to assess the impact of uncertainty on both individual components and on the system.
